Non-linear dependences in finance

The thesis is composed of three parts. Part I introduces the mathematical and statistical tools that are relevant for the study of dependences, as well as statistical tests of Goodness-of-fit for empirical probability distributions. I propose two extensions of usual tests when dependence is present in the sample data and when observations have a fat-tailed distribution. The financial content of the thesis starts in Part II. I present there my studies regarding the "cross-sectional" dependences among the time series of daily stock returns, i.e. the instantaneous forces that link several stocks together and make them behave somewhat collectively rather than purely independently. A calibration of a new factor model is presented here, together with a comparison to measurements on real data. Finally, Part III investigates the temporal dependences of single time series, using the same tools and measures of correlation. I propose two contributions to the study of the origin and description of "volatility clustering": one is a generalization of the ARCH-like feedback construction where the returns are self-exciting, and the other one is a more original description of self-dependences in terms of copulas. The latter can be formulated model-free and is not specific to financial time series. In fact, I also show here how concepts like recurrences, records, aftershocks and waiting times, that characterize the dynamics in a time series can be written in the unifying framework of the copula.

==> p2c1-correlation_matrices.tex <==

\section{Correlations}
The covariance is a symmetric, positive semi-definite bilinear operator acting on random variables.
It is a scalar product in probability spaces, 
and can be treated in the frameworks of linear algebra and matrix theory.
In this sense, the variance is a quadratic norm, 
and in fact defines the natural Euclidean distance.

The correlation (def p. ...) is the covariance of centered and rescaled variables, 
and it takes values in [-1,1].
It requires the existence and knowledge of the expected value and variance of each variable.

Quadratic loss function : linear force (springs) --> quadratic elastic (deformation) energy, 
                          nucleon-nucleon interactions --> quadratic potential, 
                          linear return covariances --> quadratic portfolio risk (variance)


                          
\subsection{Sample correlations}
Sample estimates of expectation values are obtained by averaging over realizations,
with the underlying assumption that the time average converges to the ensemble average (ergodicity).


Let $\Ret$ denote the $(T\times N)$ matrix whose lines are independent realizations of a random vector $\vect{\ret}$.
We assume that there are no missing values in the series.

The computation of the sample covariances 
\begin{equation}\label{eq:samp_cov}
	\overline\Sigma=\frac{1}{T}\left(\Ret-\frac{1}{T}\vect{1}\vect{1}^\dagger\Ret\right)^\dagger\left(\Ret-\frac{1}{T}\vect{1}\vect{1}^\dagger\Ret\right)=\frac{1}{T}\Ret^\dagger\left(\mathds{1}_{T}-\frac{1}{T}\vect{1}\vect{1}^\dagger\right)\Ret
\end{equation}
involves first the determination of the sample means $\frac{1}{T}\vect{1}^\dagger\Ret$.
Sample correlations are then obtained by normalizing the diagonal elements to 1, as
\[
	\overline\rhoP_{\ij}=\frac{\overline\Sigma_{\ij}}{\sqrt{\overline\Sigma_{ii}\overline\Sigma_{j\!j}}}
\]
It thus relies on a preliminary measurement of $\vect{\overline \ret}$ and $\diag(\overline\Sigma)$,
the later being potentially very noisy as a sum of squared values.

Quand l'esperance et la variance de $g(X)$ sont connus, l'estimateur du coefficient de Pearson correspondant est moins bruite.
$\betaB$, $\rhoS$ et $\tauK$ n'ont pas besoin de pr\'e-estimer ces quantit\'es !!!
%Quand $g(x)=\sign(x)$ avec des variables symetriques, alors $\esp{g(X)}=\med{X}$ et $\var{g(X)}=1$,
%et on n'a besoin que de pr\'e-estimer la m\'ediane (qui est tr\`e bas moment, quasiment pas bruit\'e).
%Quand $g(x)=\cdf{X}(x)$, alors carr\'ement $\esp{g(X)}=\frac12$ et $\var{g(X)}=\frac{1}{3}$, et on n'a rien besoin de pr\'e-estimer !




                          
\subsection{Random Matrix Theory}
\nomenclature{RMT}{Random matrix theory}%

\cite{laloux1999noise,laloux2000random,potters2005financial,potters2009financial,bouchaud2003theory}

Wishart matrices (flat time average):
for independent, and for arbitrary covariance.

Exponentially weighted moving time average (EMA)





%\section{Nested single factor model}
\section{Hierarchical models and trees}
Nested single factor model, see Appendix~\ref{chap:APXnested}.

\section{Flat factor models}
Statistical vs Known factors; 
Endogenous vs Exogenous factors;
Who cares for the residuals ? 
%\subsection{Econometrician's regressions: CAPM, APT, Fama-French, Ross, etc.}
%\nomenclature{CAPM}{Capital asset pricing model}%
%\nomenclature{APT}{Arbitrage pricing theory}%

\subsection{Principal Components Analysis}
%\subsection{Orthogonalizing the residuals}

\section{Beyond linear correlations}
Graphs and networks, structural models

